Target PCA: Transfer Learning Large Dimensional Panel Data

This paper develops a novel method to estimate a latent factor model for a large target panel with missing observations by optimally using the information from auxiliary panel data sets. We refer to our estimator as target-PCA. Transfer learning from auxiliary panel data allows us to deal with a large fraction of missing observations and weak signals in the target panel. We show that our estimator is more efficient and can consistently estimate weak factors, which are not identifiable with conventional methods. We provide the asymptotic inferential theory for target-PCA under very general assumptions on the approximate factor model and missing patterns. In an empirical study of imputing data in a mixed-frequency macroeconomic panel, we demonstrate that target-PCA significantly outperforms all benchmark methods.

==> estimation_loading.tex <==
\section{"Interchanged" Target-PCA Method}
\label{sec: estimator loadings first}
In this section, we propose an improved target-PCA estimator for latent factors. By adding an auxiliary step of estimating loadings before extracting latent factors, we can relax the strong assumption on observation pattern made in Section \ref{sec: assumption factor first} and get rid of the regime with slower convergence rate in Theorem \ref{thm: consistency F factor first}. Due to the fact that factors and loadings are equivalent in conventional factor models, this method can also be viewed as an "interchanged" version of target-PCA method. 

We present this improved target-PCA estimator and provide assumptions and general distribution theory for it.


\subsection{Estimator} \label{sec: estimator loading first}
Similar with Section \ref{sec: estimator factor first}, we first combine the partially observed data $Y$ with fully observed panel $X$ as $Z:= [X, \sqrt{\gamma}Y]$, which can be written as
$$
\begin{aligned}
Z = F \Phi^\top + \varepsilon, \quad \text{where}\ &\Phi := [\Lam; \sqrt{\gamma}\beta] \in \R^{(N+M)\times k}, \\
&\varepsilon := [e,\sqrt{\gamma}\eps] \in \R^{T\times (N+M)}.
\end{aligned}
$$




\subsection{Assumptions}
We still consider the setting where $M / N\rightarrow c \in [0,\infty)$ and set the target weight $\gamma = r\cdot N/M$, where $r$ is an arbitrary constant. 

\begin{assumption} \label{assump: obs pattern}
(Observation pattern) The observation matrix $W$ is independent of factor loadings and idiosyncratic errors. There exists positive constants $\alpha$ and $q$ such that $\frac{|Q_{ij}|}{T^\alpha}\geq q>0$ for any $i,j$ and $T.$ 
\end{assumption}

\begin{remark}
Assumption \ref{assump: obs pattern} is much weaker than Assumption \ref{assump: obs pattern factors first} in that it doesn't require a unified observable proportion for all $i,j.$
\end{remark}

\begin{assumption}  \label{assump: factor model}
 (Factor model) 
 \begin{enumerate}
 \item  Factors: $\forall t, \E\|F_t\|^2 \leq \bar{F} < \infty$. There exists a positive definite $k\times k$ matrix $\Sigma_F$ such that $\frac{1}{T}\sum_{t=1}^T F_t F_t^\top \overset{p}{\rightarrow} \Sigma_F$ and $\E \left\|\sqrt{T}\left(\frac{1}{T}\sum_{t=1}^T F_t F_t^\top -\Sigma_F\right)\right\|^2 \leq C$. Furthermore, $\frac{1}{|Q^Z_{ij}|} \sum_{t \in Q_{ij}^Z} F_tF_t^\top \overset{p}{\rightarrow} \Sigma_F$ and $\E \left\|\sqrt{|Q^Z_{ij}|}\left(\frac{1}{|Q^Z_{ij}|}\sum_{t \in Q^Z_{ij}} F_t F_t^\top -\Sigma_F\right)\right\|^2 \leq C$ for any $i,j.$

 \item  Factor loadings: loadings are independent of factors and errors. For any $i,j$, $\E\|\Lam_i\|^4 \leq \bar{\Lam}<\infty$, $\E\|\beta_j\|^4 \leq \bar{\beta} < \infty,$ and $\frac{1}{N}\sum_{i=1}^N\Lam\Lam^\top \overset{p}{\rightarrow}\Sigma_{\Lam}$, $\frac{1}{M}\sum_{i=1}^M\beta\beta^\top \overset{p}{\rightarrow}\Sigma_{\beta}.$ Furthermore, $\Sigma_\Phi:=\Sigma_{\Lam} + \lim\gamma\frac{M}{N}\cdot \Sigma_\beta$ is a positive definite $k\times k$ matrix.
\item  Idiosyncratic errors: there exists a positive constant $C$ such that for all $T, N$ and $M$:
\begin{enumerate}
\item $\E(e_{ti})=\E(\eps_{ti})=0, \E(e_{ti}^4) \leq C$ and $\E(\eps_{ti}^4) \leq C$;
\item $\E(e_{ti}e_{si}) = \gamma^{(e)}_{st,i}$ with $|\gamma_{st,i}^{(e)}| \leq \gamma_{st}$ and $\E(\eps_{ti}\eps_{si}) = \gamma^{(\eps)}_{st,i}$ with $|\gamma_{st,i}^{(\eps)}| \leq \gamma_{st}$ for some $\gamma_{st}$ and all $i$, $\sum_{s=1}^T \gamma_{st} \leq C$ for all $t$;
\item $\E(e_{ti}e_{tj}) = \tau_{ij,t}^{(e)}$ with $|\tau_{ij,t}^{(e)}| \leq \tau_{ij}^{(e)}$ for some $\tau_{ij}^{(e)}$ and all $t$, $\sum_{j=1}^{N} \tau_{ij}^{(e)} \leq C$ for all $i$; $\E(\eps_{ti}\eps_{tj}) = \tau_{ij,t}^{(\eps)}$ with $|\tau_{ij,t}^{(\eps)}| \leq \tau_{ij}^{(\eps)}$ for some $\tau_{ij}^{(\eps)}$ and all $t$, $\sum_{j=1}^{M} \tau_{ij}^{(\eps)} \leq C$ for all $i$; and $\E(\eps_{ti}e_{tj}) = \tau_{ij,t}^{(\eps,e)}$ with $|\tau_{ij,t}^{(\eps,e)}| \leq \tau_{ij}^{(\eps,e)}$ for some $\tau_{ij}^{(\eps,e)}$ and all $t$, $\sum_{i=1}^{M} \tau_{ij}^{(\eps,e)} \leq C$ for all $j$.
\item $\E(e_{ti}e_{sj}) = \tau_{ij,ts}^{(e)},$ and $\sum_{j=1}^N \sum_{s=1}^T|\tau_{ij,ts}^{(e)}|\leq C$ for all $i$ and $t;$ $\E(\eps_{ti}\eps_{sj}) = \tau_{ij,ts}^{(\eps)},$ and for all $i$ and $t$, $\sum_{j=1}^M \sum_{s=1}^T|\tau_{ij,ts}^{(\eps)}|\leq C$; $\E(e_{ti}\eps_{sj}) = \tau_{ij,ts}^{(\eps,e)},$ and $\sum_{j=1}^M \sum_{s=1}^T|\tau_{ij,ts}^{(\eps,e)}|\leq C$ for all $i$ and $t$.
\item For all $i,j$, $\E \Big [ \frac{1}{|Q_{ij}|^{1/2}}\sum_{t \in Q_{ij}}(\eps_{ti}\eps_{tj} - \E(\eps_{ti} \eps_{tj}))       \Big]^4 \leq C$, $\E \Big [ \frac{1}{T^{1/2}}\sum_{t =1}^T (e_{ti}e_{tj} - \E(e_{ti} e_{tj}))       \Big]^4 \leq C$ and $\E \Big [ \frac{1}{|Q_{jj}|^{1/2}}\sum_{t \in Q_{jj}}(e_{ti}\eps_{tj} - \E(e_{ti}\eps_{tj})) \Big]^4 \leq C$.
\end{enumerate}
\item  Weak dependence between factor and idiosyncratic errors: for any $(i,j),$
 \[
 \E \left\|\frac{1}{\sqrt{|Q^Z_{ij'}|}}\sum_{t \in Q^Z_{ij'}}F_t \eps_{tj} \right\|^2 \leq C \quad \text{and} \quad  \E \left\|\frac{1}{\sqrt{|Q^Z_{ij}|}}\sum_{t \in Q^Z_{ij}}F_t e_{tj} \right\|^2 \leq C,
 \]
 where $j'=j+N.$ 
 \item  Eigenvalues: the eigenvalues of $\Sigma_F \Sigma_\Phi$ are distinct.
  \end{enumerate}
\end{assumption}


\begin{assumption} \label{assump: additional assumptions} (Additional assumptions for factor estimator) 
\begin{enumerate}
 \item  $\E \Big\|\frac{\sqrt{NT}}{N^2}\sum_{i,j=1}^{N}\Lam_j\Lam_j^\top \frac{1}{T}\sum_{s=1}^T F_s\Lam_i^\top e_{si} \Big\|^2\leq C$,\\
 $\E \Big\|\frac{\sqrt{MT^\alpha}}{M^2}\sum_{i,j=1}^{M}\beta_j\beta_j^\top \frac{1}{{|Q_{ij}|}}\sum_{s\in Q_{ij}} F_s\beta_i^\top \eps_{si} \Big\|^2\leq C$, \\
 $\E \Big\|\frac{\sqrt{NT^\alpha}}{MN}\sum_{i=1}^{N}\sum_{j=1}^{M}\beta_j\beta_j^\top \frac{1}{{|Q_{jj}|}}\sum_{s\in Q_{jj}} F_s\Lam_i^\top e_{si} \Big\|^2\leq C$,\\
 $\E \Big\|\frac{\sqrt{MT^\alpha}}{MN}\sum_{i=1}^{M}\sum_{j=1}^{N}\Lam_j\Lam_j^\top \frac{1}{{|Q_{ii}|}}\sum_{s\in Q_{ii}} F_s\beta_i^\top \eps_{si} \Big\|^2\leq C$.
 \item  For any $t$, $\E \Big\|\sqrt{\frac{T}{N^3}}\sum_{i,j=1}^{N}\frac{1}{T}\sum_{s=1}^T\phi_{ij,st} [e_{si} e_{sj} - \E(e_{si}e_{sj})] \Big\|^2\leq C$ with $\phi_{ij,st} = \Lam_j\Lam_i^\top$, $\Lam_j\Lam_i^\top F_s$, $\Lam_je_{ti}$, $\E \Big\|\sqrt{\frac{T^\alpha}{M^3}}\sum_{i,j=1}^{M}\frac{1}{|Q_{ij}|}\sum_{s\in Q_{ij}}\phi_{ij,st} [\eps_{si} \eps_{sj} - \E(\eps_{si}\eps_{sj})] \Big\|^2\leq C$ with $\phi_{ij,st} = \beta_j\beta_i^\top$, $W_{ti}\beta_j\beta_i^\top F_s$, $W_{ti}\beta_j\eps_{ti}$, $\E \Big\|\sqrt{\frac{T^\alpha}{N^2M}}\sum_{i=1}^{N} \sum_{j=1}^{M}\frac{1}{|Q_{jj}|}\sum_{s\in Q_{jj}}\phi_{ij,st} [e_{si} \eps_{sj} - \E(e_{si}\eps_{sj})] \Big\|^2\leq C$ with $\phi_{ij,st} = \beta_j\Lam_i^\top$, $\beta_j\Lam_i^\top F_s,$ $W_{ti}\Lam_j\beta_i^\top F_s$, $\beta_je_{ti}$, $W_{ti}\Lam_j\eps_{ti}$.
 \item  For any $t$, $\frac{1}{M}\sum_{i=1}^M W_{ti}\beta_i \beta_i^\top \overset{p}{\rightarrow} \Sigma_{\beta,t},$ and $\Sigma_{\Phi,t}:=\Sigma_\Lam + \lim \gamma \frac{M}{N}\cdot \Sigma_{\beta,t}$ is a positive definite matrix. 
 \item  For any $t$, $\frac{1}{\sqrt{N}}\sum_{i=1}^N \Lam_i e_{ti} \overset{d}{\rightarrow}\Ncal(0,\Sigma_{\Lam e,t})$, $\frac{1}{\sqrt{M}}\sum_{i=1}^M W_{ti}\beta_i \eps_{ti} \overset{d}{\rightarrow}\Ncal(0,\Sigma_{\beta\eps,t})$ and they are asymptotically independent. Furthermore, $\Gamma_{F,t}^{\text{obs}}:=\lim\frac{M}{N}\cdot\Sigma_{\Lam e,t} + \lim(\gamma \frac{M}{N})^2\cdot \Sigma_{\beta\eps,t}. $
 \item  For any $i$ and $t$,
\[
\sqrt{T^\alpha} \begin{bmatrix}
\text{vec}(X_i) \\ \text{vec}(\mathbf{X}_t)
\end{bmatrix} 
\overset{d}{\rightarrow} \mathcal{N} \left( 0, \begin{bmatrix} \Psi_i & (\Psi_{i,t}^{\text{cov}})^\top \\ \Psi_{i,t}^{\text{cov}} & \Psi_t
\end{bmatrix} \right),
\]
where for $i=1,\cdots,N$, $X_i = \gamma\cdot \frac{1}{N}\sum_{j=1}^M \beta_j\beta_j^\top \big(\frac{1}{|Q_{jj}|}\sum_{t\in Q_{jj}}F_t F_t^\top - \frac{1}{T}\sum_{t=1}^TF_t F_t^\top\big)$, for $i=N+1,\cdots,N+M$, $X_i =  \frac{1}{N}\sum_{j=1}^N \Lam_j\Lam_j^\top \big(\frac{1}{|Q_{i'i'}|}\sum_{t\in Q_{i'i'}}F_t F_t^\top - \frac{1}{T}\sum_{t=1}^TF_t F_t^\top\big) + \gamma\cdot \frac{1}{N}\sum_{j=1}^M \beta_j\beta_j^\top \big(\frac{1}{|Q_{i'j}|}\sum_{t\in Q_{i'j}}F_t F_t^\top - \frac{1}{T}\sum_{t=1}^TF_t F_t^\top\big)$ with $i'=i-N$, and for any $t$, $\mathbf{X}_t = \frac{1}{N}\sum_{i=1}^{N}X_i\Lam_i\Lam_i^\top + \gamma\cdot \frac{1}{N}\sum_{i=1}^M X_{i+N} W_{ti}\beta_i^\top \beta_i$. 

\item For any $t$ and $j=1,\cdots,M,$ $\E\big\|\sqrt{\frac{{T^\alpha}}{N}}\sum_{i=1}^{N} (\frac{1}{|Q_{jj}|}\sum_{s\in Q_{jj}}F_sF_s^\top - \frac{1}{T}\sum_{s=1}^TF_s F_s^\top) \Lam_i e_{ti}\big\|^2\leq C$ and $\E\big\|\sqrt{\frac{{T^\alpha}}{M}}\sum_{i=1}^{M} (\frac{1}{|Q_{i}^*|}\sum_{s\in Q_i^*}F_sF_s^\top - \frac{1}{T}\sum_{s=1}^TF_s F_s^\top)W_{ti} \beta_i \eps_{ti}\big\|^2\leq C$ with $Q_{i}^*=Q_{ii}$ or $Q_{ij}.$
\end{enumerate}
\end{assumption}


\subsection{Inferential Theory}
\textbf{Consistency}  

According to the "interchanged" target-PCA method in Section \ref{sec: estimator loading first}, we plug the expression of $\tilde{\Sigma}^Z$ into $\frac{1}{N+M} \tilde{\Sigma}^Z \tilde{\Phi} = \tilde{\Phi} \tilde{D}$ to derive the expansion for factor loading estimator $\tilde{\Phi}$ as
\begin{equation} \label{equ: Phi expansion 1}
\begin{aligned}
\tilde{\Phi}_i &= \frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}  \tilde{\Phi}_j \tilde{\Sigma}_{ji}^Z \\
& = \underbrace{\frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}  \tilde{\Phi}_j  \Phi_j^\top \frac{1}{|Q^Z_{ij}|}\sum_{t\in Q^Z_{ij}} F_t F_t^\top  \Phi_i}_{H_i \Phi_i} +  \underbrace{\frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}  \tilde{\Phi}_j  \Phi_i^\top \frac{1}{|Q^Z_{ij}|}\sum_{t\in Q^Z_{ij}} F_t \veps_{tj}}_{(a)} \\
& \ \ + \underbrace{\frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}  \tilde{\Phi}_j  \Phi_j^\top \frac{1}{|Q^Z_{ij}|}\sum_{t\in Q^Z_{ij}} F_t \veps_{ti}}_{(b)} + \underbrace{\frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}  \tilde{\Phi}_j   \frac{1}{|Q^Z_{ij}|}\sum_{t\in Q^Z_{ij}} \veps_{tj} \veps_{ti}}_{(c)}.
\end{aligned}
\end{equation}
The estimated factor loading is related to the true factor loading through $\tilde{\Phi}_i = H_i \Phi_i + (a) + (b) + (c)$ up to a rotation matrix 
\[
H_i = \frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}  \tilde{\Phi}_j  \Phi_j^\top \frac{1}{|Q^Z_{ij}|}\sum_{t\in Q^Z_{ij}} F_t F_t^\top 
\]
 for index $i$. For simplicity, we denote
\begin{equation}  \label{equ: def of four terms}
\begin{aligned}
&\gamma(i,j) =\frac{1}{|Q^Z_{ij}|} \sum_{t \in Q^Z_{ij}} \E[\veps_{ti} \veps_{tj}], 
\qquad \ \ \zeta_{ij} = \frac{1}{|Q^Z_{ij}|} \sum_{t \in Q^Z_{ij}} \veps_{ti}\veps_{tj} - \gamma(i,j), \\
&\eta_{ij} = \frac{1}{|Q^Z_{ij}|} \sum_{t \in Q^Z_{ij}}  \Phi_i^\top F_t \veps_{tj}, 
\qquad \qquad \xi_{ij} = \frac{1}{|Q^Z_{ij}|} \sum_{t \in Q^Z_{ij}}  \Phi_j^\top F_t \veps_{ti},
\end{aligned}
\end{equation}
then \eqref{equ: Phi expansion 1} can be rewritten as 
\begin{equation} \label{equ: Phi expansion 2}
\tilde{\Phi}_i - H_i \Phi_i = \frac{1}{N+M} \tilde{D}^{-1} \sum_{j=1}^{N+M}   \left( \tilde{\Phi}_j \eta_{ij} + \tilde{\Phi}_j \xi_{ij} + \tilde{\Phi}_j \zeta_{ij} + \tilde{\Phi}_j \gamma(i,j) \right).
\end{equation}

Since the estimation of factors requires the same rotation matrix for all $\Phi_i$, we consider a unified rotation matrix $H$ defined as 
\[
H:= \frac{1}{N+M}\tilde{D}^{-1} \sum_{j=1}^{N+M}\tilde{\Phi}_j\Phi_j^\top \frac{1}{T}\sum_{t=1}^T F_t F_t^\top = \frac{1}{T(N+M)}\tilde{D}^{-1} \tilde{\Phi}^\top \Phi F^\top F.
\]
Theorem \ref{thm: consistency for loadings} shows the consistency result of the estimated loadings.
\begin{theorem}  \label{thm: consistency for loadings}
Define $\delta_{MT} = \min(M,T^\alpha)$. Suppose that $M / N \rightarrow c\in [0,\infty)$ and let $\gamma = r\cdot N/M$, where $r$ is a constant independent of $N,M$ and $T$. Under Assumptions \ref{assump: obs pattern},\ref{assump: factor model}, as $T,N,M \rightarrow \infty,$
\[
\delta_{MT} \left( \frac{1}{N+M}\sum_{i=1}^{N+M} \|\tilde{\Phi}_i - H\Phi_i\|^2 \right) = O_p(1),
\]
where $H = T^{-1}(N+M)^{-1}\tilde{D}^{-1}\tilde{\Phi}^\top \Phi F^\top F .$
\end{theorem}
\begin{proof}
See in Appendix B.
\end{proof} 


\vbox{}
\textbf{Asymptotic Normality}

Based on the consistency result for loading estimators, we can derive the asymptotic normality result for latent factors:
\begin{theorem}  \label{thm: asymptotic of factors}
Define $\delta_{MT} = \min(M,T^\alpha)$. Suppose that $M/ N\rightarrow c\in [0,\infty)$ and let $\gamma = r\cdot N/M$, where $r$ is a constant independent of $N,M$ and $T$. Under Assumptions \ref{assump: obs pattern},\ref{assump: factor model},\ref{assump: additional assumptions}, as $T,N,M \rightarrow \infty,$ for each $t$,
\[
\sqrt{\delta_{MT}} (\tilde{F}_t - (H^{-1})^\top F_t )  \overset{d}{\rightarrow} \Ncal \left(0, Q^\top {\Sigma}_{\Phi,t}^{-1} \left[ \text{plim}\bigg(\frac{\delta_{MT}}{M}\Gamma^{\text{obs}}_{\Phi,i}  + \frac{\delta_{MT}}{T^\alpha} \Gamma^{\text{miss}}_{F,t}\bigg)\right] {\Sigma}_{\Phi,t}^{-1} Q \right),
\]
or equivalently, 
\[
\sqrt{\delta_{MT}} (H^\top \tilde{F}_t - F_t )  \overset{d}{\rightarrow} \Ncal \left(0,  {\Sigma}_{\Phi,t}^{-1} \left[ \text{plim}\bigg(\frac{\delta_{MT}}{M}\Gamma^{\text{obs}}_{F,t}  + \frac{\delta_{MT}}{T^\alpha} \Gamma^{\text{miss}}_{F,t}\bigg)\right] {\Sigma}_{\Phi,t}^{-1}  \right),
\]
where $\Gamma^{\text{obs}}_{F,t}$ is defined in Assumption \ref{assump: additional assumptions}.4, $\Gamma^{\text{miss}}_{F,t}:=(I_k \otimes(\Sigma_\Phi^{-1} \Sigma_{F}^{-1}F_t)^\top)\Psi_t(I_k \otimes(\Sigma_\Phi^{-1} \Sigma_{F}^{-1}F_t))$ and $\Psi_t$ is defined in Assumption \ref{assump: additional assumptions}.5.
\end{theorem}
\begin{proof}
See in Appendix B.
\end{proof}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
